Fourier Theory on the Complex Plane V: Arbitrary-Parity Real Functions, Singular Generalized Functions and Locally Non-Integrable Functions

A previously established correspondence between definite-parity real functions and inner analytic functions is generalized to real functions without definite parity properties. The set of inner analytic functions that corresponds to the set of all integrable real functions is then extended to include a set of singular "generalized functions" by the side of the integrable real functions. A general definition of these generalized functions is proposed and explored. The generalized functions are introduced loosely in the spirit of the Schwartz theory of distributions, and include the Dirac delta "function" and its derivatives of all orders. The inner analytic functions corresponding to this infinite set of singular real objects are given by means of a recursion relation. The set of inner analytic functions is then further extended to include a certain class of non-integrable real functions. The concept of integral-differential chains is used to help to integrate both the normal functions and the singular generalized functions seamlessly into a single structure. It does the same for the class of non-integrable real functions just mentioned. This extended set of generalized functions also includes arbitrary real linear combinations of all these real objects. An interesting connection with the Dirichlet problem on the unit disk is established and explored.

==> packages.tex <==
% JLdL 17Apr14.
%
% These are the packages to be used for the
% _ Mathematical Physics I/II lectures.
\usepackage[brazil]{babel}
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{epsfig}
\usepackage{amsfonts}
\usepackage{color}
\definecolor{lgrey}{gray}{0.99}

